Distinct switching of chiral transport in the kagome metals KV$_3$Sb$_5$ and CsV$_3$Sb$_5$

The kagome metals AV$_3$Sb$_5$ (A=K,Rb,Cs) present an ideal sandbox to study the interrelation between multiple coexisting correlated phases such as charge order and superconductivity. So far, no consensus on the microscopic nature of these states has been reached as the proposals struggle to explain all their exotic physical properties. Among these, field-switchable electric magneto-chiral anisotropy (eMChA) in CsV$_3$Sb$_5$ provides intriguing evidence for a rewindable electronic chirality, yet the other family members have not been likewise investigated. Here, we present a comparative study of magneto-chiral transport between CsV$_3$Sb$_5$ and KV$_3$Sb$_5$. Despite their similar electronic structure, KV$_3$Sb$_5$ displays negligible eMChA, if any, and with no field switchability. This is in stark contrast to the non-saturating eMChA in CsV$_3$Sb$_5$ even in high fields up to 35 T. In light of their similar band structures, the stark difference in eMChA suggests its origin in the correlated states. Clearly, the V kagome nets alone are not sufficient to describe the physics and the interactions with their environment are crucial in determining the nature of their low-temperature state.

==> preamble.tex <==
%\pdfoutput=1
\setlength{\intextsep}{10pt}
\setlength{\textfloatsep}{5pt}

%adjust height of rows in a table
\setlength\extrarowheight{2.5pt}

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

%% ultimate commands
	
	% align environment
			\newcommand{\e}[1]{\begin{align}{#1}\end{align}}	
	
		
	% fraction
		\newcommand{\f}[2]{\frac{#1}{#2}}
		\newcommand{\tf}[2]{\tfrac{#1}{#2}}
		
	% partial differentiation
		\newcommand{\p}[2]{\frac{\partial #1}{\partial #2}}
		\newcommand{\pf}[3]{\frac{\partial #1}{\partial #2}\bigg|_{#3}}
		\newcommand{\pa}[1]{\partial_{#1}}
		
	% label equations/sections
		\newcommand{\la}[1]{\label{#1}}

	% refer to equation, section, figure, appendix
		\newcommand{\q}[1]{Eq.\ (\ref{#1})}
		\newcommand{\qq}[2]{Eqs.\ (\ref{#1})-(\ref{#2})}
		\newcommand{\s}[1]{Sec.\ \ref{#1}}
		\newcommand{\fig}[1]{Fig.\ \ref{#1}}		
		\newcommand{\app}[1]{App.\ \ref{#1}}				
		\newcommand{\tab}[1]{Tab.\ \ref{#1}}
		\newcommand{\ocite}[1]{Ref.\ \onlinecite{#1}}
		\newcommand{\cf}[1]{[cf.\ Eq.\ (\ref{#1})]}
	
				
	% brackets
		\newcommand{\brac}[1]{\left(\;#1\;\right)}
		\newcommand{\sq}[1]{\left[\;#1\;\right]}
		\newcommand{\cu}[1]{\left\{\;#1\;\right\}}

	% insert words in equation environment

		\newcommand{\iwith}{\ins{with}}
		\newcommand{\where}{\ins{where}}		
		\newcommand{\iand}{\ins{and}}
		\newcommand{\ior}{\ins{or}}
		\newcommand{\ifor}{\ins{for}}
		\newcommand{\st}{\ins{s.t.}}
		
	% sign functions
		\newcommand{\sgn}{\text{sgn}}

	% equal, approximate, proportional signs, limits
		\newcommand{\eq}{=&\;}
		\newcommand{\condeq}[1]{\as \substack{\sma{#1}\\=}\as}
		\newcommand{\condprop}[1]{\as \substack{\sma{#1}\\ \propto}\as}
		\newcommand{\limit}[1]{\substack{\text{lim}\\#1}\as}		
		\newcommand{\appr}{\approx &\;}
		\newcommand{\prop}{\propto&\;}
		\newcommand{\define}{\as\substack{\text{def}\\ \iff}\as}					
	
	% mathbb symbols
		\newcommand{\F}{\mathbb{F}}
		\newcommand{\R}{\mathbb{R}}
		\newcommand{\Z}{\mathbb{Z}}
		\newcommand{\I}{\mathbb{I}}
		\newcommand{\C}{\mathbb{C}}
		\newcommand{\N}{\mathbb{N}}		
		\newcommand{\Q}{\mathbb{Q}}				
		\newcommand{\bbs}{\mathbb{S}}
		\newcommand{\bbt}{\mathbb{T}}

		
% for review
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

% exponential 
\newcommand{\ex}{\text{exp}}
\newcommand{\pexp}{\overline{\text{exp}}}
		
		
% plane wave
	\newcommand{\eikr}{e^{i\bk \cdot \br}}
	\newcommand{\eikR}{e^{i\bk \cdot \bR}}
	\newcommand{\emikr}{e^{-i\bk \cdot \br}}
	\newcommand{\emikR}{e^{-i\bk \cdot \bR}}	

% divergence,curl,laplacian
\newcommand{\na}{\nabla}
\newcommand{\nai}{\nabla_i}
\newcommand{\naj}{\nabla_j}
\newcommand{\nak}{\nabla_k}
\newcommand{\nal}{\nabla_l}
\newcommand{\diverge}{\nabla \cdot}
\newcommand{\curl}{\nabla \times}
\newcommand{\lap}{\nabla^2}
\newcommand{\nabr}{\nabla_{\boldsymbol{r}}}
\newcommand{\nabk}{\nabla_{\boldsymbol{k}}}
\newcommand{\nabkp}{\nabla_{\boldsymbol{k}'}}

%fundamental constants
\newcommand{\bohr}{\mu_{\sma{B}}}
\newcommand{\gfac}{g_{\sma{0}}}
\newcommand{\lmt}{l^{\mt}}
\newcommand{\lmf}{l^{\text{-}4}}
\newcommand{\lmo}{l^{\mo}}




% specific to geometric_orbital
\newcommand{\om}{orbital moment }
\newcommand{\omm}{orbital moment}
\newcommand{\zf}{Zilberman-Fischbeck }
\newcommand{\checkgp}{\check{g}^{\sma{\perp}}}
\newcommand{\btperp}{$BT_{\sma{\perp}}$}
\newcommand{\bise}{Bi$_2$Se$_3$}



% c creation operators

\newcommand{\cdagk}{\dg{c}_{\bk}}
\newcommand{\ck}{\pdg{c}_{\bk}}
\newcommand{\cdagksig}{\dg{c}_{\bk,\sigma}}
\newcommand{\cksig}{\pdg{c}_{\bk,\sigma}}
\newcommand{\cdagkup}{c^\dagger_{\boldsymbol{k}\uparrow}}
\newcommand{\cdagkdo}{c^\dagger_{\boldsymbol{k}\downarrow}}
\newcommand{\ckup}{\pdg{c}_{\boldsymbol{k} \uparrow}}
\newcommand{\ckdo}{\pdg{c}_{\boldsymbol{k} \downarrow}}

\newcommand{\cdag}[1]{c^{\scriptscriptstyle{\dagger}}_{\scriptstyle{#1}}}
\newcommand{\cnod}[1]{c_{\scriptstyle{#1}}}


\newcommand{\cdj}{c^{\scriptscriptstyle{\dagger}}_{\scriptstyle{j \sigma}}}
\newcommand{\cnj}{c_{\scriptstyle{j' \sigma'}}}


% f creation operator

\newcommand{\fsig}{\pdg{f}_{\sigma}}
\newcommand{\fdagsig}{\dg{f}_{\sigma}}
\newcommand{\fup}{\pdg{f}_{\uparrow}}
\newcommand{\fdagup}{\dg{f}_{\uparrow}}
\newcommand{\fdo}{\pdg{f}_{\downarrow}}
\newcommand{\fdagdo}{\dg{f}_{\downarrow}}


%levi Cevita
\newcommand{\levi}[1]{\epsilon_{#1}}


%spin symbols
\newcommand\nup{\hat{n}_{f\uparrow}}
\newcommand\ndo{\hat{n}_{f\downarrow}}
\newcommand\avenup{{n}_{f\uparrow}}
\newcommand\avendo{{n}_{f\downarrow} }

% energies with varepsilon
\newcommand{\var}{\varepsilon}
%\newcommand{\var}[1]{\varepsilon_{#1}}
\newcommand{\efu}{\varepsilon_{\scriptscriptstyle{F}}^{\scriptscriptstyle{\uparrow}}}
\newcommand{\efd}{\varepsilon_{\scriptscriptstyle{F}}^{\scriptscriptstyle{\downarrow}}}
\newcommand{\ef}{\varepsilon_{\scriptscriptstyle{f}}}
\newcommand{\EF}{E_{\scriptscriptstyle{F}}}
\newcommand{\ek}{\varepsilon_{\boldsymbol{k}}}
\newcommand{\eF}{\varepsilon_{\scriptscriptstyle{F}}}
\newcommand{\enk}{\varepsilon_{n,\bk}}




% space

\newcommand\as{\;\;\;\;}
\newcommand\ass{\;\;\;\;\;\;\;\;}


\newcommand\Wline[2]{ \pdg{\W}_{\sma{#1 \leftarrow #2}}}


%hat operators

\newcommand{\hn}{\hat{n}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hN}{\hat{N}}
\newcommand{\hO}{\hat{O}}
\newcommand{\hPi}{\hat{{\Pi}}}
\newcommand{\hpsi}{\hat{{\psi}}}
\newcommand{\hphi}{\hat{{\phi}}}
\newcommand{\hrho}{\hat{{\rho}}}
\newcommand{\hsigma}{\hat{{\sigma}}}
	%hatted operators with dagger
	\newcommand{\dhpsi}{\dg{\hat{{\psi}}}}
	\newcommand{\dhphi}{\dg{\hat{{\phi}}}}


%hatted bold symbols
\newcommand{\hbp}{\hat{\bp}}
\newcommand{\hbr}{\hat{\br}}
\newcommand{\hbv}{\hat{\bv}}
\newcommand{\hbx}{\hat{\bx}}
\newcommand{\bhp}{\boldsymbol{\hat{p}}}
\newcommand{\hbA}{\hat{\bA}}
\newcommand{\hbB}{\hat{\bB}}
\newcommand{\hbJ}{\hat{\bJ}}
\newcommand{\hbP}{\hat{\bP}}
\newcommand{\hbpi}{\hat{\boldsymbol{\pi}}}
\newcommand{\hbPi}{\hat{\boldsymbol{\Pi}}}


%bold symbols

\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bkp}{\boldsymbol{k}_{\sma{\perp}}}
\newcommand{\bkpar}{\bk_{\parallel}}
\newcommand{\bkone}{\boldsymbol{k_1}}
\newcommand{\bktwo}{\boldsymbol{k_2}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\brp}{\boldsymbol{r}_{\sma{\perp}}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bze}{\boldsymbol{0}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bcalf}{\boldsymbol{\calf}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvarpi}{\boldsymbol{\varpi}}
\newcommand{\bdeltapar}{\boldsymbol{\delta}_{\sma{\parallel}}}
\newcommand{\bna}{\boldsymbol{\nabla}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}



%\mathfrak
\newcommand{\frake}{\mathfrak{e}}
\newcommand{\frako}{\mathfrak{o}}
\newcommand{\frakt}{\mathfrak{t}}
\newcommand{\fraks}{\mathfrak{s}}
\newcommand{\frakr}{\mathfrak{r}}
\newcommand{\mx}{\mathfrak{X}}
\newcommand{\mxx}{\mathfrak{X}^x}
\newcommand{\mxy}{\mathfrak{X}^y}
\newcommand{\bmx}{\bar{M}_x}


\newcommand{\orb}{\boldsymbol{\mathfrak{A}}}
\newcommand{\lutt}{\boldsymbol{\mathfrak{L}}}



%tilde
\newcommand{\tbPi}{\tilde{\bPi}}
\newcommand{\tPi}{\tilde{\Pi}}
\newcommand{\txi}{\tilde{\xi}}
\newcommand{\tbv}{\tilde{\bv}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\tbmx}{\tilde{\bmx}}
\newcommand{\tmxx}{\tilde{\mx}^x}
\newcommand{\tmxy}{\tilde{\mx}^y}
\newcommand{\tmx}{\tilde{\mx}}
\newcommand{\tH}{\tilde{H}}
\newcommand{\tbsigma}{\tilde{\bsigma}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\tilu}[1]{\tilde{u}_{#1}}
\newcommand\tilX{\tilde{X}}
\newcommand\tilZ{\tilde{Z}}
\newcommand\tilGamma{\tilde{\Gamma}}
\newcommand\tilU{\tilde{U}}

%calligraphic
\newcommand{\calL}{{\cal L}}
\newcommand{\W}{{\cal W}}
\newcommand{\A}{{\cal A}}


% equal signs
\newcommand\kzeq{\;\stackrel{\mathclap{\normalfont\mbox{$\sma{\bar{k}_z}$}}}{=}\;}

%breve 
\newcommand{\breveg}{\breve{g}}


% symmetry operators
\newcommand{\inv}{\mathfrak{i}}
\newcommand{\mir}{\mathfrak{r}}
\newcommand\glide{\mathfrak{g}}
\newcommand\rot{\mathfrak{c}}
\newcommand\scr{\mathfrak{s}}
\newcommand\tra{\mathfrak{t}}


\newcommand{\calti}{{\cal T}_{\sma{\cal I}}}
\newcommand{\gdel}{g_{\boldsymbol{\delta}}}
\newcommand{\pgdel}{\pdg{g}_{\boldsymbol{\delta}}}
\newcommand{\bmz}{\bar{M}_z}
\newcommand{\calbmx}{{\cal \bar{M}}_x}
\newcommand{\calgdel}{\pdg{\breve{g}}_{\sma{\bdelta}}}
\newcommand{\brevegdel}{\pdg{\breve{g}}_{\sma{\bdelta}}}
\newcommand{\brevebmx}{\breve{\bar{M}}_x}
\newcommand{\uit}{U_{\sma{\cali T}}}
\newcommand{\utg}{U_{\sma{Tg \bdelta}}}
\newcommand{\ut}{U_{\sma{T}}}
\newcommand{\ug}{U_{\sma{g \bdelta}}}
\newcommand{\ubmx}{U_{\sma{\bmx}}}
\newcommand{\utbmz}{U_{\sma{T\bmz}}}
\newcommand{\calug}{\calg_{\sma{\bdelta}}}
\newcommand{\caluit}{\calu_{\sma{\cali T}}}
\newcommand{\caltgdel}{\breve{T}_{\sma{g \bdelta}}}
\newcommand{\brevetgdel}{\breve{T}_{\sma{g \bdelta}}}
\newcommand{\brevetbmx}{\breve{T}_{\sma{\bmx}}}
\newcommand{\hattbmx}{\hat{T}_{\sma{\bmx}}}
\newcommand{\brevetbmz}{\breve{T}_{\sma{\bmz}}}
\newcommand{\breveti}{\breve{T}_{\sma{\cali}}}
\newcommand{\caltbmz}{\calt_{\sma{\bmz}}}
\newcommand{\caltbmx}{\calt_{\sma{\bmx}}}
\newcommand{\calut}{\calu_{\sma{T}}}
\newcommand{\hatgdel}{\pdg{\hat{g}}_{\sma{\bdelta}}}
\newcommand{\hatTg}{\pdg{\hat{T}}_{\sma{g\bdelta}}}
\newcommand\csixdel{C_{\sma{6,\bdelta}}}
\newcommand\brevecsixdel{\breve{C}_{\sma{6,\bdelta}}}
\newcommand\cthreedel{C_{\sma{3,\bdelta}}}
\newcommand\brevecthreedel{\breve{C}_{\sma{3,\bdelta}}}
\newcommand\hatcthreedel{\hat{C}_{\sma{3,\bdelta}}}
\newcommand\cthreetwodel{C_{\sma{3,2\bdelta}}}
\newcommand\brevecthreetwodel{\breve{C}_{\sma{3,2\bdelta}}}
\newcommand\brevectwothreedel{\breve{C}_{\sma{2,3\bdelta}}}
\newcommand\ctwothreedel{C_{\sma{2,3\bdelta}}}
\newcommand\hatcsixdel{\hat{C}_{\sma{6,\bdelta}}}
\newcommand\ucsixdel{U_{\sma{C_6,\bdelta}}}
\newcommand\cndel{C_{\sma{n,\bdelta}}}
\newcommand\cbarndel{C_{\sma{\bar{n},\bdelta}}}
\newcommand\ucndel{U_{\sma{C_n,\bdelta}}}
\newcommand\hatcndel{\hat{C}_{\sma{n,\bdelta}}}
\newcommand\brevecndel{\breve{C}_{\sma{n,\bdelta}}}
\newcommand\brevectwotwodel{\breve{C}_{\sma{2,2\bdelta}}}
\newcommand\brevecfourdel{\breve{C}_{\sma{4,\bdelta}}}
\newcommand\brevectwodel{\breve{C}_{\sma{2,\bdelta}}}


% vectors and matrices
\newcommand{\vectwo}[2]{\begin{pmatrix} {#1}\\{#2} \end{pmatrix}}
\newcommand{\matrixtwo}[4]{\begin{pmatrix} #1 & #2 \\ #3 & #4 \end{pmatrix}}
\newcommand{\diagmatrix}[2]{\begin{pmatrix} #1 & 0 \\ 0 & #2 \end{pmatrix}}
\newcommand{\matrixthree}[9]{\begin{pmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \\ #7 & #8 & #9 \end{pmatrix}}


% Pauli matrices
\newcommand{\szero}{\sigma_{\sma{0}}}
\newcommand{\sx}{\sigma_{\sma{1}}}
\newcommand{\sy}{\sigma_{\sma{2}}}
\newcommand{\sz}{\sigma_{\sma{3}}}
\newcommand{\tzero}{\tau_{\sma{0}}}
\newcommand{\tx}{\tau_{\sma{1}}}
\newcommand{\ty}{\tau_{\sma{2}}}
\newcommand{\tz}{\tau_{\sma{3}}}



% parafermion operators
\newcommand{\gt}{\gamma_{\sma{2}}}
\newcommand{\gth}{\gamma_{\sma{3}}}
\newcommand{\gfo}{\gamma_{\sma{4}}}
\newcommand{\gfi}{\gamma_{\sma{5}}}
\newcommand{\gj}{\gamma_{\sma{j}}}
\newcommand{\gtj}{\gamma_{\sma{2j}}}
\newcommand{\gtjpo}{\gamma_{\sma{2j+1}}}
\newcommand{\gtjpt}{\gamma_{\sma{2j+2}}}
\newcommand{\gtjmo}{\gamma_{\sma{2j-1}}}
\newcommand{\gtL}{\gamma_{\sma{2L}}}
\newcommand{\gtLpo}{\gamma_{\sma{2L+1}}}
\newcommand{\gtLpt}{\gamma_{\sma{2L+2}}}
\newcommand{\gtLmo}{\gamma_{\sma{2L-1}}}
\newcommand{\gtLmt}{\gamma_{\sma{2L-2}}}
\newcommand{\gtLmth}{\gamma_{\sma{2L-3}}}
\newcommand{\gtLmfo}{\gamma_{\sma{2L-4}}}


% insert text in equation
\newcommand{\ins}[1]{\;\;\;\;\text{#1}\;\;\;\;}


%momentum parallel and perpendicular
\newcommand{\kpar}{\boldsymbol{k}_{{\shortparallel}}}
\newcommand{\Dpar}{D^{g}_{{\shortparallel}}}
\newcommand{\kper}{k_{\perp}}


% Cnv 
\newcommand{\ctv}{C_{3v}}
\newcommand{\cfv}{C_{4v}}
\newcommand{\csv}{C_{6v}}
\newcommand{\cnv}{C_{nv}}


%C_n Time-reversal
\newcommand{\cnt}{C_n {\cal T}}
\newcommand{\cn}{C_n}
\newcommand{\cfour}{C_4}
\newcommand{\cs}{C_6}
\newcommand{\ct}{C_3}
\newcommand{\cst}{C_6{\cal T}}
\newcommand{\cft}{C_4{\cal T}}
\newcommand{\ctt}{C_2{\cal T}}


% average 
\newcommand{\ave}[1]{\langle\,#1\,\rangle}



%inverse Angstroms and Angstroms
\newcommand{\invA}{\mathrm{\AA^{\scriptscriptstyle{-1}}}}
\newcommand{\ang}{\mathrm{\AA}}

% Lagrangian
\newcommand{\lag}{{\mathscr{L}}}


% green's function
\newcommand{\green}{{\mathscr{G}}}

% Cauchy principal value
\newcommand{\prin}{{\mathscr{P}}}

% imaginary and real parts
\newcommand{\imag}{{\mathscr{I}}}
\newcommand{\real}{{\mathscr{R}}}


%total differentiation
\newcommand{\totaldif}[2]{\frac{ d #1}{d #2}}

% calligraphic font
\newcommand{\cala}{{\cal A}}
\newcommand{\calb}{{\cal B}}
\newcommand{\calc}{{\cal C}}
\newcommand{\cald}{{\cal D}}
\newcommand{\cale}{{\cal E}}
\newcommand{\calf}{{\cal F}}
\newcommand{\calg}{{\cal G}}
\newcommand{\calh}{{\cal H}}
\newcommand{\tcalh}{\tilde{\cal H}}
\newcommand{\cali}{{\cal I}}
\newcommand{\calj}{{\cal J}}
\newcommand{\calk}{{\cal K}}
\newcommand{\call}{{\cal L}}
\newcommand{\calm}{{\cal M}}
\newcommand{\caln}{{\cal N}}
\newcommand{\calo}{{\cal O}}
\newcommand{\calp}{{\cal P}}
\newcommand{\calq}{{\cal Q}}
\newcommand{\calr}{{\cal R}}
\newcommand{\cals}{{\cal S}}
\newcommand{\calt}{{\cal T}}
\newcommand{\calu}{{\cal U}}
\newcommand{\calv}{{\cal V}}
\newcommand{\calw}{{\cal W}}
\newcommand{\calx}{{\cal X}}
\newcommand{\caly}{{\cal Y}}
\newcommand{\calz}{{\cal Z}}

% mathscript font
\newcommand{\scra}{{\mathscr A}}
\newcommand{\scrb}{{\mathscr B}}
\newcommand{\scrc}{{\mathscr C}}
\newcommand{\scrd}{{\mathscr D}}
\newcommand{\scre}{{\mathscr E}}
\newcommand{\barscre}{\bar{\mathscr E}}
\newcommand{\scrf}{{\mathscr F}}
\newcommand{\scrg}{{\mathscr G}}
\newcommand{\scrh}{{\mathscr H}}
\newcommand{\tscrh}{\tilde{\mathscr H}}
\newcommand{\scri}{{\mathscr I}}
\newcommand{\scrj}{{\mathscr J}}
\newcommand{\scrk}{{\mathscr K}}
\newcommand{\scrl}{{\mathscr L}}
\newcommand{\scrm}{{\mathscr M}}
\newcommand{\scrn}{{\mathscr N}}
\newcommand{\scro}{{\mathscr O}}
\newcommand{\scrp}{{\mathscr P}}
\newcommand{\scrq}{{\mathscr Q}}
\newcommand{\scrr}{{\mathscr R}}
\newcommand{\scrs}{{\mathscr S}}
\newcommand{\scrt}{{\mathscr T}}
\newcommand{\scru}{{\mathscr U}}
\newcommand{\scrv}{{\mathscr V}}
\newcommand{\scrw}{{\mathscr W}}
\newcommand{\scrx}{{\mathscr X}}
\newcommand{\scry}{{\mathscr Y}}
\newcommand{\scrz}{{\mathscr Z}}


%Gamma matrices
\newcommand{\gam}[1]{\Gamma_{#1}}

%determinant
\newcommand{\de}[1]{\text{det}[\;#1\;]}

%trace
\newcommand{\tr}{\text{Tr}}




\newcommand{\noi}[1]{\noindent (#1)}
\newcommand{\imp}{\;\;\Rightarrow\;\;}
\newcommand{\mo}{\text{-}1}
\newcommand{\mt}{\text{-}2}
\newcommand{\minus}{\text{-}}
\newcommand{\oneover}[1]{\tfrac{1}{#1}}


% A command for inner product and bras and kets
\newcommand{\braket}[2]{\big\langle #1 \big| #2 \big\rangle}
\newcommand{\ketbra}[2]{\big|  #1  \big\rangle \big\langle #2 \big| }
\newcommand{\braopket}[3]{\big\langle #1 \big| #2 \big| #3 \big\rangle}
\newcommand{\bra}[1]{\big\langle#1\big|}
\newcommand{\ket}[1]{\big|#1\big\rangle}
\newcommand{\bigket}[1]{\bigl|#1\bigr\rangle}
\newcommand{\textket}[1]{|#1\rangle}
  %double bras and kets
	\newcommand{\dbraket}[2]{\big\langle\big\langle #1 \big| #2 \big\rangle \big\rangle}
  \newcommand{\dketbra}[2]{\big|  #1  \big\rangle\big\rangle \big\langle \big\langle #2 \big| }
  \newcommand{\dbraopket}[3]{\big\langle \big\langle #1 \big| #2 \big| #3 \big\rangle \big\rangle}
  \newcommand{\dket}[1]{\big|#1\big\rangle \big\rangle}
  \newcommand{\dbra}[1]{\big\langle \big\langle#1\big|}
  \newcommand{\dexp}[1]{\big\langle\big\langle #1 \big\rangle \big\rangle}



% Various bracketing commands
\newcommand{\of}[1]{\!\left(#1\right)}
\newcommand{\sqof}[1]{\left[#1\right]}
\newcommand{\cuof}[1]{\left\{#1\right\}}

% commutator and anticommutator
\newcommand{\comm}[2]{\left[#1,#2\right]}
\newcommand{\anticomm}[2]{\left\{#1,#2\right\}}
% sum on nearest neighbor bonds
\newcommand{\bond}{\left\langle i, j \right\rangle}
%\newcommand{\bondsum}{\sum_{\left\langle i, j \right\rangle}}
\newcommand{\nbond}{\left\langle\left\langle i, j \right\rangle\right\rangle}
% 1/2
\newcommand{\half}{\frac{1}{2} }
\newcommand{\thalf}{\tfrac{1}{2} }
% simplifies using the up and down arrows to denote spin
\newcommand{\up}{\uparrow}
\newcommand{\down}{\downarrow}
% Absolute value  
\newcommand{\abs}[1]{\left|#1\right|}

% Roman functions for real and imaginary parts
\newcommand{\re}{\mathrm{Re}}
\newcommand{\im}{\mathrm{Im}}


%Expectation values
\newcommand{\expect}[1]{\left\langle#1\right\rangle}
\newcommand{\pdag}{\phantom{\dagger}}
\newcommand{\pdg}[1]{{#1}^{\phantom{\dagger}}}

\newcommand{\bkap}{\bar{\glide}}
\newcommand{\bchi}{\bar{\chi}}
\newcommand{\baeta}{\bar{\eta}}
\newcommand{\lin}{\notag \\}



\newcommand{\ab}{\alpha\beta}
\newcommand{\deli}{\Delta^{-1}}


\newcommand{\ra}{{R\,\alpha}}
\newcommand{\rax}{{R+\vec{x}\,\alpha}}

\newcommand{\rb}{{R'\,\beta}}
\newcommand{\rarb}{{R\,\alpha};R'\,\beta}
\newcommand{\zth}{\mathbb{Z}_3}


\newcommand{\xin}{x_{\tex{inv}}}
\newcommand{\low}{L$\ddot{\text{o}}$wdin\;}
\newcommand{\tex}[1]{\sma{\text{#1}}}











\newcommand{\kf}{k_{\scriptscriptstyle{F}}}

\newcommand{\bfk}{\boldsymbol{k}}
\newcommand{\bfq}{\boldsymbol{q}}



\newcommand{\bpm}{\begin{pmatrix}}
\newcommand{\epm}{\end{pmatrix}}
\newcommand{\nk}{n_{\boldsymbol{k}'}}
\newcommand{\dk}{\Delta_{\boldsymbol{k}'}}
\newcommand{\Dk}{\Delta_{\boldsymbol{k}}}
\newcommand{\tk}{\tilde{k}}
\newcommand{\tkp}{\tilde{k}'}
\newcommand{\bal}{\begin{align}}
\newcommand{\Ainv}{\mathrm{\AA^{\scriptscriptstyle{-1}}}}

\newcommand{\V}{V_{\text{eff}}}
\newcommand{\si}{\;\text{sin}\,}
\newcommand{\ta}{\;\text{tan}\,}
\newcommand{\co}{\;\text{\text{cos}}\,}
\newcommand{\te}{t_{\text{eff}}}
\newcommand{\ep}{\bar{\epsilon}}



\newcommand{\braa}[1]{\left\langle#1\right|_{\scriptscriptstyle{A}}}
\newcommand{\brab}[1]{\left\langle#1\right|_{\scriptscriptstyle{B}}}

\newcommand{\dg}[1]{#1^{\scriptstyle{\dagger}}}
\newcommand{\bof}[1]{\boldsymbol{#1}}
\newcommand{\sma}[1]{\scriptscriptstyle{#1}}
\newcommand{\po}{{\sma{+}} 1}



\newcommand{\noc}{n_{\sma{{occ}}}}
\newcommand{\ntot}{n_{\sma{{tot}}}}

\newtheorem{definition}{Definition}[section]
